Context Matters: Leveraging Contextual Features for Time Series Forecasting

Time series forecasts are often influenced by exogenous contextual features in addition to their corresponding history. For example, in financial settings, it is hard to accurately predict a stock price without considering public sentiments and policy decisions in the form of news articles, tweets, etc. Though this is common knowledge, the current state-of-the-art (SOTA) forecasting models fail to incorporate such contextual information, owing to its heterogeneity and multimodal nature. To address this, we introduce ContextFormer, a novel plug-and-play method to surgically integrate multimodal contextual information into existing pre-trained forecasting models. ContextFormer effectively distills forecast-specific information from rich multimodal contexts, including categorical, continuous, time-varying, and even textual information, to significantly enhance the performance of existing base forecasters. ContextFormer outperforms SOTA forecasting models by up to 30% on a range of real-world datasets spanning energy, traffic, environmental, and financial domains.

==> figures/Experiments/graph.tex <==
\begin{figure}[h!]
    \centering
    
    % First Subfigure
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{tikzpicture}[node distance=2cm, auto]
            % Nodes
            \node[circle, draw, minimum size=1cm] (X) at (0, 0) {\(\mX\)};
            \node[circle, draw, below of=X, minimum size=1cm] (W) {\(\mC\)};
            
            % Coordinate for midpoint
            \coordinate (midpoint) at ($(X)!0.5!(W)$);
            
            % Node for Y placed to the right of the midpoint
            \node[circle, draw, right of=midpoint, minimum size=1cm, node distance=2cm] (Y) {\(\hat{\mX}\)};
            \node[circle, draw, right of=Y, minimum size=1cm] (Z) {$\Tilde{\mX}$};

            % Arrows with labels
            \draw[->] (X) -- node[above] {} (Y);
            \draw[->] (W) -- node[below] {} (Y);
            \draw[->] (Y) -- node[above] {} (Z);
        \end{tikzpicture}
        \caption{Context-aware Forecasting Model}
        \label{fig:sub2}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{tikzpicture}[node distance=2cm, auto]
            % Nodes
            \node[circle, draw, minimum size=1cm, yshift=2cm] (A) at (0, 0){\(\mX\)};
            \node[circle, draw, right of=A, minimum size=1cm] (B) {\(\hat{\mX}\)};
            \node[circle, draw, right of=B, minimum size=1cm] (C) {$\Tilde{\mX}$};

            % Arrows with labels
            \draw[->] (A) -- node[above] {} (B);
            \draw[->] (B) -- node[above] {} (C);
        \end{tikzpicture}
        \caption{Context-agnostic Forecasting Model}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    % Second Subfigure
    

    \caption{\textbf{Graphical models for forecasting}: The figures represent the graphical models for the two different forecasting approaches. In the context-aware, the forecast $\hat{\mX}$ follows from both the history $\mX$ and context $\mC$, while for the context-agnostic model, $\hat{\mX}$ is dependent only on history $\mX$.}
    \label{fig:graph}
\end{figure}

==> sections/tables/main_results.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{2}
\begin{sc}
\begin{tabular}{lccccccccccc} %cc
\hline
\multicolumn{2}{c}{\Large{Model}}                                        
& \multicolumn{4}{c}{\Large{PatchTST}}    
& \multicolumn{4}{c}{\Large{iTransformer}}        
& \multicolumn{2}{c}{\Large{Baseline}}            
\\

\multicolumn{2}{c}{Method}                                            
& \multicolumn{2}{c}{Context-agnostic}
& \multicolumn{2}{c}{Context-aware}    
& \multicolumn{2}{c}{Context-agnostic}
& \multicolumn{2}{c}{Context-aware}
& \multicolumn{2}{c}{Chronos}                  
%& \multicolumn{2}{c}{TimesFM}
\\

\rule{0pt}{-10ex} Dataset   & $T$                     
& MAE                                          
& MSE                                          
& MAE                                          
& MSE                                           
& MAE                                          
& MSE                                          
& MAE                                          
& MSE  
% & MAE                                          
% & MSE                                          
& MAE                                          
& MSE \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AQ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[HTML]{FFCCC9} 
\cellcolor[HTML]{FFCCC9}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9}48} 
&$0.573 $   
&$0.770 $      
&\textbf{0.524}                                           
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9} \textbf{0.674} } 
&$0.577 $   
&$0.771$      
&\underline{0.540}                                  
&\multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9}\underline{0.696 }  }  
&0.591
& 0.825
% & 0.611
% &  0.847
\\ 
\rowcolor[HTML]{FFCCC9} 
\multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}Air Quality} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9}96} 
&$0.622$                                      
&$0.901$                                      
& \textbf{0.572}                                               
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9}\textbf{0.802} } 
&$0.631 $                                      
&$0.919$                                      
& \underline{0.591}                                     
    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9}\underline{0.813}   }   & 0.665
& 0.973
% & 0.660
% & 1.001
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Elec %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[HTML]{CBCEFB} 
\cellcolor[HTML]{CBCEFB}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}48} 
&\underline{0.029}                                      
&\underline{0.037}                                    
& \textbf{0.024}                                                  
& \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}\textbf{0.027} } 
&$0.038 $                                      
&$0.059$                                      
& $0.031 $                                     
& \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}$0.039 $ }    & 0.039
&0.060
% & 0.084
% &  0.249  
\\
\rowcolor[HTML]{CBCEFB} 
\multirow{-2}{*}{\cellcolor[HTML]{CBCEFB}Electricity} & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}96} 
&$0.039 $                                      
&$0.042 $                                      
& \underline{0.029}                                                 
& \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}\underline{0.040}} 
&$0.047 $                                      
&$0.083$                                      
& \textbf{0.028}                                     
& \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}\textbf{0.033}    }
& 0.044
& 0.063
% &0.065
% & 0.187 
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Traffic %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[HTML]{FFCE93} 
\cellcolor[HTML]{FFCE93} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}48} 
&$1.101 $                                      
&$3.520 $                                             
& $0.866 $                                     
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}$2.946 $} 
&$1.022$                                      
&$3.265$                                      
& \underline{0.847}                                    
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\underline{2.868}  }                                             
&0.909
& 4.231
% &\textbf{0.795}
% &\textbf{2.516}
\\
\rowcolor[HTML]{FFCE93} \multirow{-2}{*}{\cellcolor[HTML]{FFCE93}Traffic}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}96} 
&$1.084 $                                      
&$3.415 $                                             
& 0.845                                    
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}$2.767 $} 
&$1.025 $                                      
&$3.165$                                      
& \underline{0.830}                                     
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.766 }   
& 0.990
& 4.724
% &\textbf{0.758}
% & \textbf{2.428}
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Stores %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[HTML]{9AFF99}  \cellcolor[HTML]{9AFF99} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}48} 
&$0.123 $                                      
&$0.238 $                                          
& \underline{0.115}                                      
& \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\underline{0.228}} 
&$0.130 $                                      
&$0.257$                                          
& 0.124                                              
& \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}0.257 }     
& 0.141
& 0.302
% & \textbf{0.114}
% &  \textbf{0.215}
\\
\rowcolor[HTML]{9AFF99} \multirow{-2}{*}{\cellcolor[HTML]{9AFF99}Retail} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}96} 
& $0.139 $                               
&$0.291 $                                     
&\textbf{0.128}                                     
& \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{0.265}} 
& $0.145 $                               
&$0.309$                                     
&$0.143 $                                           
&  \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}$0.310 $  }  
& 0.169
& 0.382
% & \underline{0.131}
% & \underline{0.274} 
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Bitcoin %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}48} 
&  0.854
& 1.231
&  0.821
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7} 1.192} 
&  0.832
& 1.177
&  \underline{0.810} 
&\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7} \underline{1.153}}
& 0.919
&1.224
% & \textbf{0.724}
% & \textbf{0.921}
\\
\rowcolor[HTML]{FFFFC7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFC7}Bitcoin}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}96} 
&  0.971
&  1.561
&  \textbf{0.948}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7} \textbf{1.537}} 
& 0.992
& 1.650
&  \underline{0.951}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}  \underline{1.547}}
& 1.008
& 1.613
% & 0.973
% & 1.573
\\ \hline
\end{tabular}
\end{sc}
}
\caption{\textbf{ContextFormer enhances forecasting accuracy:} Comparison of PatchTST and transformer, with and without the additional ContextFormer (CF) architecture on forecasting time series for the aforementioned datasets with a fixed lookback length $L=96$ and forecast lengths $T\in\{48,96\}$. The best results for both the metrics in each row are highlighted in \textbf{bold}, while the send best results are \underline{underlined}. Notably, the context-aware forecasters outperform all the context-agnostic models, including Chronos, a large pre-trained base model for all the rows on both metrics.The results for our context-aware models are comparable to TimesFM, a SOTA foundational model for time-series forecasting that takes in contextual metadata.}
\label{tab:main}
\end{table}
